Learning Structure-Aware Representations of Dependent Types

Agda is a dependently-typed programming language and a proof assistant, pivotal in proof formalization and programming language theory. This paper extends the Agda ecosystem into machine learning territory, and, vice versa, makes Agda-related resources available to machine learning practitioners. We introduce and release a novel dataset of Agda program-proofs that is elaborate and extensive enough to support various machine learning applications -- the first of its kind. Leveraging the dataset's ultra-high resolution, which details proof states at the sub-type level, we propose a novel neural architecture targeted at faithfully representing dependently-typed programs on the basis of structural rather than nominal principles. We instantiate and evaluate our architecture in a premise selection setup, where it achieves promising initial results, surpassing strong baselines.

==> Makefile <==
TEX_DEPS=fancyhdr.sty algorithmic.sty algorithm.sty agda-example.tex
TEX_FLAGS=-pdf -file-line-error -halt-on-error -interaction=nonstopmode -shell-escape

default: main.pdf

all: main.pdf aitp.pdf


%.pdf: %.tex $(TEX_DEPS)
	latexmk $(TEX_FLAGS) $<

nix::
	nix-shell --run "make"

%.tex: %.lagda
	agda --latex --latex-dir=. $<

%.json: %.lagda
	agda2train $<

agda-example: agda-example.tex
json-example: agda-example.json

clean:
	rm -f *.aux main.pdf *.fls *.log *.fdb_latexmk *.out \
  agda-example.tex agda-example.json

.PHONY=default nix-paper agda-example json-exampleclean

